Toxic Memes: A Survey of Computational Perspectives on the Detection and Explanation of Meme Toxicities

Internet memes, channels for humor, social commentary, and cultural expression, are increasingly used to spread toxic messages. Studies on the computational analyses of toxic memes have significantly grown over the past five years, and the only three surveys on computational toxic meme analysis cover only work published until 2022, leading to inconsistent terminology and unexplored trends. Our work fills this gap by surveying content-based computational perspectives on toxic memes, and reviewing key developments until early 2024. Employing the PRISMA methodology, we systematically extend the previously considered papers, achieving a threefold result. First, we survey 119 new papers, analyzing 158 computational works focused on content-based toxic meme analysis. We identify over 30 datasets used in toxic meme analysis and examine their labeling systems. Second, after observing the existence of unclear definitions of meme toxicity in computational works, we introduce a new taxonomy for categorizing meme toxicity types. We also note an expansion in computational tasks beyond the simple binary classification of memes as toxic or non-toxic, indicating a shift towards achieving a nuanced comprehension of toxicity. Third, we identify three content-based dimensions of meme toxicity under automatic study: target, intent, and conveyance tactics. We develop a framework illustrating the relationships between these dimensions and meme toxicities. The survey analyzes key challenges and recent trends, such as enhanced cross-modal reasoning, integrating expert and cultural knowledge, the demand for automatic toxicity explanations, and handling meme toxicity in low-resource languages. Also, it notes the rising use of Large Language Models (LLMs) and generative AI for detecting and generating toxic memes. Finally, it proposes pathways for advancing toxic meme detection and interpretation.

==> src/comp_approaches.tex <==

\subsection{Computational Approaches}

% TASK 1: For detecting role of entities in harmful memes:

% The task is formulated as “Given a meme and an entity, determine the role of the entity in the meme: hero vs. villain vs. victim vs. other.”
% Nandi et al 2022: Detecting the Role of an Entity in Harmful Memes: Techniques and Their Limitations
% % https://arxiv.org/pdf/2205.04402.pdf

% % The idea for this section is to expand on the latest survey (from Sharma et al 2022) (see figure below), because there has been a HUGE amount of papers published since then). We can add not only new papers and works, but also more detail regarding whether they used external knowledge or not, what kind, if they are interpretable to any degree, and if so, with what techniques... We have to harmonize Sharma's table from the figure with a table I have been working on, to determine some of the data we want to get from the approaches that have been tried. For now, I am collecting some data in this Google Doc, since I am continuously adding/taking out columns (it is not stable yet). 
% % https://docs.google.com/spreadsheets/d/1BlnxywxfP-p8TZqTL_4rbNoKwRn4ccExr1PICBSYgWg/edit?usp=sharing
% \begin{figure}
%         \centering
%         \includegraphics[width=1\linewidth]{sharma_soa.png}
%         \caption{Enter Caption}
%         \label{fig:enter-label}
%     \end{figure}
    

\begin{itemize}

% MOMENTA: A Multimodal Framework for Detecting Harmful Memes and Their Targets: https://arxiv.org/pdf/2109.05184.pdf


    \item \textbf{KERMIT \cite{grasso2024kermit}:} KERMIT (Knowledge-EmpoweRed Model In harmful meme deTection) is a novel framework that integrates external knowledge from ConceptNet into the process of identifying harmful memes. It builds a knowledge-enriched information network by combining internal meme entities with relevant external knowledge. KERMIT employs a dynamic learning mechanism using memory-augmented neural networks and attention mechanisms to identify informative knowledge for accurate classification of harmful memes. Experimental results on four benchmark datasets demonstrate that KERMIT effectively utilizes external knowledge to improve classification performance compared to several state-of-the-art baselines. \textbf{USES BACKGROUND KNOWLEDGE!}

    \item \textbf{Hate-CLIPper \cite{2022hate}:} Hate-CLIPper is an architecture that models cross-modal interactions between image and text representations using Contrastive Language-Image Pre-training (CLIP) encoders. It achieves state-of-the-art performance on the Hateful Memes Challenge (HMC) dataset and demonstrates generalizability on other meme datasets such as Propaganda Memes and TamilMemes. The interpretability of the feature interaction matrix (FIM) representation is analyzed, showing that cross-modal interactions facilitate the learning of meaningful concepts.\textbf{CROSS-MODAL IS IMPORTANT!}
    % https://arxiv.org/pdf/2210.05916.pdf

    \item \textbf{DISARM \cite{sharma2022disarm}:} DISARM (Detecting vIctimS targeted by hARmful Memes) proposes a framework for detecting harmful memes by annotating each meme with its victim(s). It uses named entity recognition and person identification to detect all entities targeted by a meme and incorporates a contextualized multimodal deep neural network for classification. Evaluation results show that DISARM significantly outperforms ten unimodal and multimodal systems, demonstrating interpretability and generalizability.

    \item \textbf{MemeFier \cite{koutlis2023memefier}:} MemeFier is a deep learning-based architecture for fine-grained classification of Internet image memes. It utilizes a dual-stage modality fusion module to capture non-trivial connections between text and image components of memes. MemeFier leverages a Transformer encoder to learn inter-modality correlations at the token level. Additionally, it considers external knowledge and background image caption supervision for improved performance. Experimental results on three benchmark datasets show competitive performance, with the approach sometimes surpassing state-of-the-art methods.

    \item  \textbf{ISSUES} \cite{burbi2023mapping}: Multimodal image-text memes are prevalent on the internet, serving as a unique form of communication that combines visual and textual elements to convey humor, ideas, or emotions. However, some memes take a malicious turn, promoting hateful content and perpetuating discrimination. Detecting hateful memes within this multimodal context is a challenging task that requires understanding the intertwined meaning of text and images. In this work, we address this issue by proposing a novel approach named ISSUES for multimodal hateful meme classification. ISSUES leverages a pre-trained CLIP vision-language model and the textual inversion technique to effectively capture the multimodal semantic content of the memes. The experiments show that our method achieves state-of-the-art results on the Hateful Memes Challenge and HarMeme datasets. The code and the pre-trained models are publicly available at https://github.com/miccunifi/ISSUES

    \item \textbf{Meme Analytical Tool Kit (MATK)} \cite{hee2023matk} ...

\end{itemize}

==> src/contextuality.tex <==


\subsection{Trend 2: Tackling Contextuality, Cultural and Background Knowledge}

The process of semiosis, which involves the interpretation of signs and symbols within a given context, is crucial for understanding internet memes, particularly in the context of identifying toxic or offensive content. Memes, characterized by their intertextuality, often reference elements from popular culture, symbols, events, or artifacts that hold significance within specific communities or affinity spaces \cite{knobel2007online}. This intertextuality renders memes highly contextual, necessitating background knowledge on various topics, including politics, current events, and cultural references, for accurate interpretation. This background knowledge, often referred to as "meme literacy" or "prior knowledge," is fundamental for comprehending the nuanced meanings embedded within memes \cite{Bi2023You}. In the realm of toxic memes, contextualization becomes even more critical. A seemingly innocuous image can take on a malicious connotation simply by altering the context in which it is presented. For instance, the Nesquik bunny, originally featured in public information and awareness campaigns, was repurposed and recontextualized into a disparaging humor meme mocking the African water crisis \cite{polli2023multimodal}. This example underscores the importance of understanding the semiotic implications of memes, where a shift in context can completely change the interpretation and impact of the content.

Recent trends in meme classification systems highlight the increasing attention put on incorporating contextual, expert, background and/or cultural background understanding to enhance effectiveness and interpretability. For instance, Kougia et al. \cite{kougia2023memegraphs} propose utilizing scene graphs and knowledge graphs to represent memes, integrating structured representations and interactions between internal entities and external knowledge. Their Transformer-based architecture consistently improves classification performance compared to models relying solely on learned representations. Similarly, Grasso et al. \cite{Grasso2024KERMIT} introduce KERMIT, a framework that integrates external knowledge from ConceptNet into meme classification, leveraging knowledge-enriched information networks and memory-augmented neural networks to enhance classification performance. KnowMeme, developed by Shang et al. \cite{shang2021knowmeme}, addresses the challenge of detecting offensive memes by utilizing a knowledge-enriched graph neural network incorporating human commonsense knowledge. By effectively capturing implicit meanings and cross-modal relations in memes, KnowMeme achieves significant performance gains compared to baseline methods, highlighting the importance of incorporating external knowledge in accurately detecting offensive meme posts on social media platforms. Moreover, Zhong et al. \cite{zhong2022combining} propose MeBERT, a model for meme classification that enhances semantic representation by incorporating conceptual information from external knowledge bases. Through the design of a concept-image attention module and deep convolution tensor fusion module, MeBERT outperforms existing techniques, demonstrating the value of integrating expert knowledge for improved classification. These studies collectively emphasize the critical role of expert and cultural background knowledge in enhancing the interpretability and effectiveness of meme classification systems, ultimately contributing to a safer and more responsible online environment.


____
Memes often derive their meaning from contextual cues and cultural references, which presents a challenge in accurately interpreting and analyzing them without considering their broader socio-cultural contexts.
Resources containing human knowledge into a machine-readable format to enhance the performance and explainability of meme analysis. It will explore existing resources that contain relevant background knowledge, such as Internet Meme Knowledge Graph (IMKG), Know Your Meme (KYM), Global Project Against Hate and Extremism (GPAHE), and Anti-Defamation League (ADL). The paper will survey these resources and propose ideas on how they can be leveraged in machine readable ways to improve contextual understanding and analysis of memes within their socio-cultural contexts.

    
    \item \textbf{IMKG:} (No description provided)

\subsection{Resources for Background Knowledge of Toxicity and Hate}

\begin{itemize}
    \item \textbf{GPAHE: Global Project Against Hate and Extremism:} The Global Project Against Hate and Extremism provides a comprehensive database on global far-right and extremist symbols. This database serves as a crucial resource for combating hate and extremism, enabling various organizations worldwide to recognize and address far-right hate movements efficiently. Access the database to combat hate and extremism effectively. 
    % Extremist groups exploit symbols to amplify their messages, spread hateful ideologies, and instill fear in targeted communities. These symbols also function as markers of membership and solidarity, akin to gang insignias, making them effective recruitment and intimidation tools. World’s largest database on global far-right and extremist symbols. Originally introduced in mid-2023, this recent expansion has more than doubled the number of entries cataloged, now with over 750 symbols and identifiers, enhancing its effectiveness as a tool to combat hate and extremism. It's a pivotal resource for tech companies, governments, law enforcement agencies, militaries, and civil society organizations worldwide, enabling them to recognize and address far-right hate movements efficiently

    
 \item \textbf{Hate on Display™ Hate Symbols Database:} Curated by the Anti-Defamation League (ADL), this database provides a comprehensive collection of symbols commonly used by white supremacist and hate groups. It serves as a valuable resource for understanding hate ideology and extremism, offering real-world examples of these symbols in various contexts such as signage, clothing, and tattoos. Emphasizing careful interpretation, the database acknowledges that symbols may carry multiple meanings and contexts. Users are encouraged to contribute new symbols, ensuring the database remains relevant and up-to-date. Each entry offers a detailed description of the symbol or group, including any relevant alternate names or variations. Users can easily search for specific symbols or explore different categories to gain insights into the world of hate symbolism and extremism. The database categorizes its entries into several sections for easy navigation and reference. These sections include:

    \begin{itemize}
        \item \textbf{General Hate Symbols:} Featuring symbols frequently used by hate groups, such as the Confederate Flag, Burning Cross, and Swastika.
        
        \item \textbf{Hate Acronyms/Abbreviations:} Listing acronyms and abbreviations commonly associated with hate ideology.
        
        \item \textbf{Hate Group Symbols/Logos:} Highlighting symbols and logos adopted by specific hate groups, such as Aryan Brotherhood of Texas, Aryan Nations, and Patriot Front.
        
        \item \textbf{Hate Slogans/Slang Terms:} Featuring slogans and phrases commonly used by hate groups." These phrases often convey supremacist ideologies or discriminatory messages.
        
        \item \textbf{Ku Klux Klan Symbols:} Showcasing symbols specifically associated with the Ku Klux Klan, such as the Burning Cross, Ku Klux Klan robes, and the Triangular Klan Symbol.
        
        \item \textbf{Neo-Nazi Symbols:} Presenting symbols commonly used by neo-Nazi groups, including the Swastika, SS Bolts, and the Nazi Party Flag.
        
        \item \textbf{Numeric Hate Symbols:} Including numeric codes and symbols used to represent hate-related concepts. These numeric symbols may reference historical events or promote extremist beliefs.
        
        \item \textbf{Racist Hand Signs:} Highlighting hand gestures associated with hate groups. These gestures are often used as symbols of allegiance to supremacist ideologies or as provocative gestures intended to intimidate or offend.
        
        \item \textbf{Racist Prison Gang Symbols:} Displaying symbols utilized by racist prison gangs, such as the 211 Crew, Aryan Brotherhood of Texas, and the Aryan Circle.
    \end{itemize}

    \item \textbf{Símbolos del Odio. Análisis Simbología del Odio\footnote{\url{https://alternativasindical.es/wp-content/uploads/ponencia-Sr.-Docal.pdf}}} \cite{docal2012simbolos}: Authored by David Docal Gil, a Subinspector of the Spanish National Police Force and a Professor at the Center for Advanced Police Studies, this resource is a practical and didactic manual enriched with research findings, validated data, and expert opinions. It systematically examines hate symbols, stressing their accurate interpretation for comprehending their significance, especially in digital spaces and sports stadiums where dissemination is widespread. Furthermore, it explores contemporary strategies of neo-fascist movements, drawing parallels to historical contexts. Serving as a comprehensive investigation into hate discourse propagation toward marginalized groups, it underscores the need for law enforcement agencies to address the absence of clear legislation regarding hate symbols in Spain. Available online, it aims to serve as a reference guide for understanding and combating hate ideology, with plans for continuous updates and expansions to enhance its usefulness. It is organized into five sections:
    \begin{itemize}
        \item \textbf{Acronyms Catalog:} Provides a list of 23 acronyms and numerals commonly used by various extremist groups, particularly neo-Nazis, shedding light on their historical contexts and contemporary usage within extremist circles.
        
        \item \textbf{Flag Catalog:} Features detailed descriptions and images of 25 flags commonly associated with extremist groups, particularly neo-Nazis. Textual descriptions offer insights into the flags' origins, symbolism, and associations with extremist ideologies.
        
        \item \textbf{Symbols Catalog:} Presents a curated selection of 25 symbols commonly used by neo-Nazi groups, including pictographic imagery. Each symbol entry includes at least one image for visual recognition, accompanied by textual descriptions explaining their historical origins, ideological significance, and contemporary usage within extremist circles.
        
        \item \textbf{Salutes:} Outlines 4 common salutations frequently utilized by neo-Nazi groups to venerate their idols, flags, and symbols. Each salute is accompanied by a visual pictogram for easy identification and described in detail, providing contextual information.
        
        \item \textbf{Aesthetics:} Delves into 3 distinct clothing brands commonly associated with neo-Nazi subculture: "CONSDAPLE," "WERWOLF," and "THREE STROKE." Provides insights into the historical backgrounds and ideological underpinnings of these brands, highlighting their connections to far-right extremism.
    \end{itemize}


    \item \textbf{Spanish Interior Ministry Database}: The Ministry of Interior plans to establish a shared database on extremist symbols to combat hate crimes \cite{diariodesevilla2019}. This database will include information on symbols used by radical groups, such as those with homophobic, racist, antisemitic, or Islamophobic connotations. Expected to be operational by the end of 2019, the database aims to address the increase in hate crimes in recent years in Spain as part of the Action Plan against Hate Crimes announced by the Ministry of Interior.

    \item Digital Activism Toolkit. General hub for relevant tools: \url{https://en.hive-mind.community/tools}


\end{itemize}


\textbf{Lighthouse} is a hate symbol-tracking tool developed by the City of Edmonton in Canada in partnership with the Anti-Defamation League (ADL) to address the issue of hate symbols, such as graffiti, which undermine residents' sense of well-being and safety.  It aims to combat hate on a local level and address the underlying issues leading to anti-racism behaviors. The project aimed to create an approachable and highly usable tool that provides current hate symbol knowledge to frontline employees and decision-makers. Lighthouse utilizes the "Hate on Display" database, integrated into the tool's products. Lighthouse consists of three interconnected tools:

\begin{itemize}
    \item \textbf{Lantern}: Mobile phone application designed for data collection. Frontline workers utilize Lantern to capture photographs of potential hate symbols encountered in their communities. Each image is securely stored along with metadata detailing the time and location of the photograph, ensuring comprehensive data capture.
    
    \item \textbf{Gallery}: Web application tailored for the analysis of the collected data. This platform facilitates the review and categorization of images uploaded through Lantern. Leveraging the extensive Hate on Display™ Hate Symbol Database provided by the ADL, Gallery plays a pivotal role in the identification and categorization of hate symbols, enabling a nuanced understanding of the prevalence and distribution of such symbols.
    
    \item \textbf{Watch}: Dynamic dashboard that consolidates and visualizes the data collected through Lantern and analyzed via Gallery. Watch provides decision-makers with actionable insights by highlighting hate symbols, their spatial and temporal distribution, and emerging patterns.
\end{itemize}

Showcased at the Anti-Defamation League's Never is Now Summit in New York in November 2022, the tool garnered attention from various organizations, including the FBI. 






% \subsection{Resources for Automatic Understanding of Memes}

% https://github.com/digitalmethodsinitiative/4cat 4CAT is a research tool that can be used to analyse and process data from online social platforms. Its goal is to make the capture and analysis of data from these platforms accessible to people through a web interface, without requiring any programming or web scraping skills. Our target audience is researchers, students and journalists interested using Digital Methods in their work.

% In 4CAT, you create a dataset from a given platform according to a given set of parameters; the result of this (usually a CSV or JSON file containing matching items) can then be downloaded or analysed further with a suite of analytical 'processors', which range from simple frequency charts to more advanced analyses such as the generation and visualisation of word embedding models.

% 4CAT has a (growing) number of supported data sources corresponding to popular platforms that are part of the tool, but you can also add additional data sources using 4CAT's Python API. The following data sources are currently supported actively and can be used to collect data with 4CAT:

% 4chan and 8kun
% BitChute
% Reddit
% Telegram
% Tumblr
% Twitter API v2 (Academic and regular tracks)
% The following platforms are supported through other tools, with which you can collect data to import data into 4CAT for analysis:

% Instagram, TikTok, 9gag, Imgur, LinkedIn, Parler, Douyin and Twitter (via Zeeschuimer)
% Facebook and Instagram (via CrowdTangle exports)
% A number of other platforms have built-in support that is untested, or requires e.g. special API access. You can view the data sources in our wiki or review the data sources' code in the GitHub repository. It is also possible to import your own CSV files into 4CAT for analysis.

% \textbf{MATK: The Meme Analytical Tool Kit \cite{hee2023matk}:} The Meme Analytical Tool Kit (MATK) is an open-source toolkit designed to support existing meme datasets and multimodal models. It aims to assist researchers and engineers in training and reproducing these models for meme classification tasks, while also providing analysis techniques to gain insights into their strengths and weaknesses. MATK enables the reproduction, evaluation, and comparison of multimodal models using fair benchmarks and settings. Access MATK at: \url{https://github.com/Social-AI-Studio/MATK}.

==> src/issues_trends.tex <==



\subsection{Using LLMs and Generative AI for Toxic Memes}


% \subsection{Generative AI, Large Language Models (LLMs) and Prompt Engineering, Adversarial Attacks}

    % \item \textbf{Reasoning with Large Language Models (LLMs):} Lin et al. propose a method for detecting harmful memes by conducting abductive reasoning with LLMs \cite{Lin2023Beneath}. They emphasize advanced reasoning over multimodal information to unveil harmful memes, employing a generative framework to distill multimodal reasoning knowledge from LLMs for better fusion and fine-tuning. This approach achieves superior performance in harmful meme detection tasks by considering both textual and visual modalities.

The emergence of Large Language Models (LLMs) and generative artificial intelligence (AI) has provided new avenues for detecting and interpreting toxic memes. These advanced models offer capabilities for understanding implicit meanings and context in multimodal content, thereby addressing the challenges posed by harmful memes. Below are some recent works that leverage LLMs and generative AI for toxic meme detection and interpretation:

\begin{itemize}
    \item \textbf{Multimodal Reasoning with LLMs}: In \cite{Lin2023Beneath}, LLMs are employed for abductive reasoning to detect harmful memes. A novel generative framework is proposed to distill multimodal reasoning knowledge from LLMs and conduct lightweight fine-tuning. The approach outperforms state-of-the-art methods in harmful meme detection, demonstrating the efficacy of reasoning-based approaches.
    
    \item \textbf{Explainable Detection with LLMs}: \cite{lin2024towards} explores the use of multimodal debate between LLMs for explainable harmful meme detection. By facilitating a debate between LLMs, the model gains insights into the context and implicit meanings of memes, leading to more interpretable results and a deeper understanding of meme content.
    
    \item \textbf{Multimodal Generative Framework}: In \cite{jain2023generative}, a unified Multimodal Generative framework (MGex) is proposed for detecting cyberbullying in memes. This framework reframes the multitasking problem of meme detection as a multimodal text-to-text generation problem, achieving competitive performance against baselines and state-of-the-art models.
    
    \item \textbf{Analysis of Text-to-Image Models}: \cite{qu2023unsafe} focuses on demystifying the generation of unsafe images and hateful memes from Text-to-Image models. The study assesses the proportion of unsafe images generated by advanced Text-to-Image models and evaluates the potential of generating hateful meme variants, highlighting risks associated with model misuse.
    
    \item \textbf{Zero-Shot Hateful Meme Detection}: \cite{Zhu2022Multimodal} explores hateful meme detection in a zero-shot setting using a deep generative framework called Target-Aware Multimodal Enhancement (TAME). The results demonstrate significant improvements in performance, highlighting the potential of generative frameworks for zero-shot meme detection tasks.
    
    \item \textbf{Correction of Hate Speech}: \cite{van2023detecting} proposes a method for detecting and correcting hate speech in multimodal memes using a large visual language model. By leveraging the capabilities of LLMs, the model achieves effective detection and correction of hate speech, contributing to the mitigation of online toxicity.
    
    \item \textbf{Emotion Analysis with GPT Models}: \cite{Wang2023gpt} investigates the capability of GPT models to analyze the emotions of memes. By analyzing meme content using GPT models, the authors provide insights into the emotional content and context conveyed through memes, highlighting the potential of LLMs for emotion analysis tasks.
    
    \item \textbf{Proactive Generation Analysis}: \cite{wu2023proactive} explores the proactive generation of unsafe images from Text-To-Image models using benign prompts. By studying the generation process, the study highlights potential risks associated with model misuse and emphasizes the importance of implementing safety measures.
    
    \item \textbf{Performance Review of Vision-Language Models}: \cite{zhao2023review} provides a comprehensive review of vision-language models and their performance on the Hateful Memes Challenge. The authors analyze the effectiveness of different models and techniques for detecting hateful memes, providing valuable insights for future research in this domain.
\end{itemize}


These recent works demonstrate the potential of LLMs and generative AI in detecting and interpreting toxic memes. By leveraging advanced reasoning and multimodal fusion techniques, these models offer promising avenues for improving meme detection and combating online toxicity.


==> src/old_Task_datasey.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}
% \usepackage{longtable}
% Note: It may be necessary to compile the document several times to get a multi-page table to line up properly

\begin{longtable}{|p{1cm}|p{1cm}|p{.2cm}|p{1cm}|p{1cm}|p{1cm}|p{1cm}|p{1cm}|p{1cm}|}
\hline
\textbf{Toxicity term} &
  \textit{\textbf{Dataset}} &
  \multicolumn{1}{l|}{\textbf{Magnitude}} &
  \textbf{Derived from} &
  \textbf{Computational Task} &
  \textbf{Language} &
  \textbf{Subtask classifications} &
  \textbf{Labels} &
  \textbf{Task definition} \\ \hline
\endfirsthead
%
\endhead
%
 &
   &
   &
   &
   &
   &
  abusive &
  yes/no &
  binary \\ \cline{7-9} 
 &
   &
   &
   &
   &
   &
  vulgarity &
  yes/no &
  binary \\ \cline{7-9} 
 &
   &
   &
   &
   &
   &
  sentiment classification &
  positive, neutral, negative &
  single-label multi-class \\ \cline{7-9} 
 &
   &
   &
   &
   &
   &
  sarcasm &
  yes/no &
  binary \\ \cline{7-9} 
\multirow{-5}{*}{abusive} &
  \multirow{-5}{*}{\textit{BanglaAbuseMeme \cite{das2022bangla}}} &
  \multirow{-5}{*}{4043} &
  \multirow{-5}{*}{Google Image, Bing, pages and groups from Facebook and Instagram} &
  \multirow{-5}{*}{\textbf{abusive meme detection}} &
  \multirow{-5}{*}{Bengali, mix-code with English} &
  target community &
  gender, religion, national origin, individual, political, social sub-groups, others &
  single-label multi-class \\ \hline
 &
   &
   &
   &
   &
   &
  bullying &
  bully, non-bully &
  binary \\ \cline{7-9} 
 &
   &
   &
   &
   &
   &
  sentiment &
  positive, neutral, negative &
  single-label multi-class \\ \cline{7-9} 
 &
   &
   &
   &
   &
   &
  emotion &
  joy, sadness, fear, surprise, anger, disgust, anticipation, trust, ridicule &
  single-label multi-class \\ \cline{7-9} 
 &
   &
   &
   &
   &
   &
  sarcasm &
  yes/no &
  binary \\ \cline{7-9} 
\multirow{-5}{*}{cyberbullying} &
  \multirow{-5}{*}{\textit{MultiBully \cite{maity2022multitask}}} &
  \multirow{-5}{*}{5854} &
  \multirow{-5}{*}{Twitter,  Reddit} &
  \multirow{-5}{*}{\textbf{cyberbullying meme detection}} &
  \multirow{-5}{*}{hindi, code-mix} &
  harmfulness degree &
  very harmful, partially harmful, harmless &
  single-label multi-class \\ \hline
 &
   &
   &
   &
   &
   &
  bullying &
  bully, non-bully &
  binary \\ \cline{7-9} 
 &
   &
   &
   &
   &
   &
  sentiment &
  positive, neutral, negative &
  single-label multi-class \\ \cline{7-9} 
 &
   &
   &
   &
   &
   &
  emotion &
  joy, sadness, fear, surprise, anger, disgust, anticipation, trust, ridicule &
  single-label multi-class \\ \cline{7-9} 
 &
   &
   &
   &
   &
   &
  sarcasm &
  yes/no &
  binary \\ \cline{7-9} 
 &
   &
   &
   &
   &
   &
  harmfulness degree &
  very harmful, partially harmful, harmless &
  single-label multi-class \\ \cline{7-9} 
 &
   &
   &
   &
   &
   &
  textual explanation &
  textual rationales (highlighted words or phrases) &
   \\ \cline{7-9} 
\multirow{-7}{*}{cyberbullying} &
  \multirow{-7}{*}{\textit{MultiBully-Ex \cite{jha2024meme}}} &
  \multirow{-7}{*}{3222} &
  \multirow{-7}{*}{MultiBully \cite{maity2022multitask}} &
  \multirow{-7}{*}{\textbf{cyberbullying meme explanation}} &
  \multirow{-7}{*}{hindi, code-mix} &
  visual explanation &
  fg & 
   \\ \hline
 &
   &
   &
   &
   &
   &
  hate speech &
  yes/no &
  binary \\ \cline{7-9} 
 &
   &
   &
   &
   &
   &
  targeted &
  yes/no &
  binary \\ \cline{7-9} 
 &
   &
   &
   &
   &
   &
  profanity &
  yes/no &
  binary \\ \cline{7-9} 
\multirow{-4}{*}{derogatory} &
  \multirow{-4}{*}{\textit{Derogatory Facebook-Meme \cite{bhowmick2022multimodal}}} &
  \multirow{-4}{*}{650} &
  \multirow{-4}{*}{Facebook} &
  \multirow{-4}{*}{\textbf{derogatory meme detection}} &
  \multirow{-4}{*}{english, hindi, mixed languages} &
  negative sentiment &
  yes/no &
  binary \\ \hline
disinformation &
  \textit{DisinfoMeme \cite{qu2022disinfomeme}} &
  1170 &
  Facebook, related to either BLM, veganism or the pandemic &
  \textbf{disinformation meme detection} &
  english &
  disinformation &
  yes/no &
  binary \\ \hline
fake/misattribution &
  \textit{FAME dataset \cite{jabiyev2020game}} &
  1000 &
  DuckDuckGo plus Snopes, FactCheck, and PolitiFact &
  \textbf{fake meme detection} &
  english &
  fake/misattribution &
  fake, real &
  binary \\ \hline
harmful &
  \textit{Ext-Harm-P \cite{sharma2022disarm}} &
  4446 &
  Harm-P &
  \textbf{harmful reference detection} &
  english &
  harmfulness of reference of social entity &
  harmful, harmless &
  binary \\ \hline
 &
   &
   &
   &
   &
   &
  harmfulness degree &
  very harmful, partially harmful, harmless &
  single-label multi-class \\ \cline{7-9} 
\multirow{-2}{*}{harmful} &
  \multirow{-2}{*}{\textit{Harm-P \cite{pramanick2021momenta}}} &
  \multirow{-2}{*}{3552} &
  \multirow{-2}{*}{Google Image Search, Reddit, Facebook, and Instagram} &
  \multirow{-2}{*}{\textbf{harmful meme detection}} &
  \multirow{-2}{*}{english} &
  target &
  individual, community, organization, society &
  single-label multi-class \\ \hline
 &
   &
   &
   &
   &
   &
  harmfulness degree &
  very harmful, partially harmful, harmless &
  single-label multi-class \\ \cline{7-9} 
\multirow{-2}{*}{harmful} &
  \multirow{-2}{*}{\textit{Harm-C (aka HarMeme) \cite{pramanick2021detecting}}} &
  \multirow{-2}{*}{3544} &
  \multirow{-2}{*}{Google Image Search, Reddit, Facebook, and Instagram} &
  \multirow{-2}{*}{\textbf{harmful meme detection}} &
  \multirow{-2}{*}{english} &
  target &
  individual, community, organization, society &
  single-label multi-class \\ \hline
harmful &
  \textit{HVVMemes \cite{sharma2022findings}} &
  7000 &
  Harm-C \cite{pramanick2021detecting\}, Harm-P \cite{pramanick2021momenta\} &
  \textbf{entity roles in harmful memes} &
  english &
  annotated entity's role &
  hero, villain, victim, other &
  single-label multi-class \\ \hline
 &
   &
   &
   &
   &
   &
  hate speech &
  yes/no &
  binary \\ \cline{7-9} 
 &
   &
   &
   &
   &
   &
  direction (of hate) &
  directed hate,  undirected hate &
  binary \\ \cline{7-9} 
\multirow{-3}{*}{hateful} &
  \multirow{-3}{*}{\textit{CrisisHateMM \cite{bhandari2023crisishatemm}}} &
  \multirow{-3}{*}{4700} &
  \multirow{-3}{*}{Twitter, Facebook, Reddit memes related to Russia-Ukraine conflict} &
  \multirow{-3}{*}{\textbf{hateful meme detection}} &
  \multirow{-3}{*}{english} &
  target (of directed hate) &
  individual, community, organization &
  single-label multi-class \\ \hline
hateful &
  \textit{Hate Speech in Pixels \cite{sabat2019hate}} &
  5030 &
  Google Images, Reddit &
  \textbf{hateful meme detection} &
  english &
  hate speech &
  yes/no &
  binary \\ \hline
hateful &
  \textit{Facebook Hateful Memes (HM) \cite{Kiela2020}} &
  9540 &
  Artificially constructed from stock photos and designed layouts &
  \textbf{hateful meme detection} &
  english &
  hate speech &
  yes/no &
  binary \\ \hline
 &
   &
   &
   &
   &
   &
  attack type &
  dehumanizing, inferiority, inciting violence, mocking, contempt, slurs, exclusion &
  multi-label multi-class \\ \cline{7-9} 
\multirow{-2}{*}{hateful} &
  \multirow{-2}{*}{\textit{Fine grained HM (aka WOAH-2021) \cite{mathias2021findings}}} &
  \multirow{-2}{*}{9540} &
  \multirow{-2}{*}{Facebook Hateful Memes (HM) \cite{Kiela2020}} &
  \multirow{-2}{*}{\textbf{fine-grained hateful meme detection}} &
  \multirow{-2}{*}{english} &
  protected category &
  religion, race, sex, nationality, disability &
  multi-label multi-class \\ \hline
hateful &
  \textit{\begin{tabular}[c]{@{}l@{}}HatReD (Hateful meme\\ with Reasons Dataset) \cite{hee2023decoding\}\end{tabular}} &
  3228 &
  Fine grained HM \cite{mathias\} &
  \textbf{hateful meme explanation} &
  english &
  - &
  human-provided explanations of hate &
  \textbf{conditional generation task)} \\ \hline
hateful &
  \textit{Innopolis Hateful Memes \cite{Badour2022Hateful}} &
  23000 &
  memedroid, twitter, duckduckgo &
  \textbf{hateful meme detection} &
  english &
  hate speech &
  yes/no &
  binary \\ \hline
hateful &
  \textit{Indian Political Memes (IPM) \cite{rajput2022hate}} &
  1218 &
  Google images &
  \textbf{hateful meme detection} &
  hinglish &
  hate speech &
  non-offensive, hate-inducing, satirical &
  single-label multi-class \\ \hline
 &
   &
   &
   &
   &
   &
  misogyny &
  yes/no &
  binary \\ \cline{7-9} 
 &
   &
   &
   &
   &
   &
  aggressiveness &
  yes/no &
  binary \\ \cline{7-9} 
\multirow{-3}{*}{misogynous} &
  \multirow{-3}{*}{\textit{Misogynistic-MEME (MM) \cite{gasparini2022benchmark}}} &
  \multirow{-3}{*}{800} &
  \multirow{-3}{*}{\begin{tabular}[c]{@{}l@{}}Facebook, Twitter, Instagram, and\\ Reddit)\end{tabular}} &
  \multirow{-3}{*}{\textbf{misogynous meme detection}} &
  \multirow{-3}{*}{english} &
  irony &
  yes/no &
  binary \\ \hline
 &
   &
   &
   &
   &
   &
  misogyny &
  yes/no &
  binary \\ \cline{7-9} 
\multirow{-2}{*}{misogynous} &
  \multirow{-2}{*}{\textit{Multimedia Misogyny Datase (MAMI) \cite{fersini2022semeval}}} &
  \multirow{-2}{*}{10000} &
  \multirow{-2}{*}{\begin{tabular}[c]{@{}l@{}}Twitter, Reddit, 9GaG, Knowyourmeme and\\ Imgur\end{tabular}} &
  \multirow{-2}{*}{\textbf{misogynous meme detection}} &
  \multirow{-2}{*}{english} &
  misogynous attack type &
  general misogyny/shaming/stereotype/objectification/violence &
  multi-label multi-class \\ \hline
 &
   &
   &
   &
   &
   &
  offensiveness &
  yes/no &
  binary \\ \cline{7-9} 
 &
   &
   &
   &
   &
   &
  explicitness (of offensiveness) &
  implict, explicit &
  binary \\ \cline{7-9} 
\multirow{-3}{*}{offensive} &
  \multirow{-3}{*}{\textit{Emoffmeme \cite{kumari2023emoffmeme}}} &
  \multirow{-3}{*}{7500} &
  \multirow{-3}{*}{Google Images} &
  \multirow{-3}{*}{\textbf{offensive meme detection}} &
  \multirow{-3}{*}{hindi} &
  sentiment classification &
  fear, neglect, irritation, rage, disgust, nervousness, shame, disappointment, envy, suffering, sadness, joy, pride, surprise &
  multi-label multi-class \\ \hline
 &
   &
   &
   &
   &
   &
  metaphorical expression &
  metaphorical/liberal &
  binary \\ \cline{7-9} 
 &
   &
   &
   &
   &
   &
  \cellcolor[HTML]{FFFFFF}metaphor type &
  text dominant, image dominant, complementary &
  single-label multi-class \\ \cline{7-9} 
 &
   &
   &
   &
   &
   &
  offensiveness degree &
  non-offensive, slight, moderate, very offensive &
  single-label multi-class \\ \cline{7-9} 
 &
   &
   &
   &
   &
   &
  sentiment &
  happiness, love, anger, sorrow, fear, hate, surprise &
  single-label multi-class \\ \cline{7-9} 
\multirow{-5}{*}{offensive} &
  \multirow{-5}{*}{\textit{MET-Meme \cite{xu2022metmeme}}} &
  \multirow{-5}{*}{10045} &
  \multirow{-5}{*}{Twitter, Weibo, Google Images, Baidu images} &
  \multirow{-5}{*}{\textbf{offensive meme detection within meme understanding}} &
  \multirow{-5}{*}{english, chinese, bilingual *scores shown are for english} &
  intention &
  interactive, expressive, purely entertaining, offensive, other &
  single-label multi-class \\ \hline
 &
   &
   &
   &
   &
   &
  sentiment &
  very positive, positive, neutral, negative, very negative &
  single-label multi-class \\ \cline{7-9} 
 &
   &
   &
   &
   &
   &
  emotion &
  sarcastic, humorous, motivation, offensive &
  multi-label multi-class \\ \cline{7-9} 
 &
   &
   &
   &
   &
   &
  sarcasm &
  not sarcastic, general, twisted meaning, very twisted &
  single-label multi-class \\ \cline{7-9} 
 &
   &
   &
   &
   &
   &
  humour &
  not funny, funny, very funny, hilarious &
  single-label multi-class \\ \cline{7-9} 
 &
   &
   &
   &
   &
   &
  offensiveness &
  not offensive, slight, very offensive, hateful offensive &
  single-label multi-class \\ \cline{7-9} 
\multirow{-6}{*}{offensive} &
  \multirow{-6}{*}{\textit{Memotion 1 \cite{sharma2020semeval}}} &
  \multirow{-6}{*}{10000} &
  \multirow{-6}{*}{Google images} &
  \multirow{-6}{*}{\textbf{offensive meme detection within meme understanding}} &
  \multirow{-6}{*}{english} &
  motivation &
  motivation/not motivational &
  binary \\ \hline
 &
   &
  \multicolumn{1}{l|}{} &
   &
   &
   &
  sentiment &
  very positive, positive, neutral, negative, very negative &
  single-label multi-class \\ \cline{7-9} 
 &
   &
  \multicolumn{1}{l|}{} &
   &
   &
   &
  emotion &
  sarcastic, humorous, motivation, offensive &
  multi-label multi-class \\ \cline{7-9} 
 &
   &
  \multicolumn{1}{l|}{} &
   &
   &
   &
  sarcasm &
  not sarcastic, general, twisted meaning, very twisted &
  single-label multi-class \\ \cline{7-9} 
 &
   &
  \multicolumn{1}{l|}{} &
   &
   &
   &
  humour &
  not funny, funny, very funny, hilarious &
  single-label multi-class \\ \cline{7-9} 
 &
   &
  \multicolumn{1}{l|}{} &
   &
   &
   &
  offensiveness &
  not offensive, slight, very offensive, hateful offensive &
  single-label multi-class \\ \cline{7-9} 
 &
   &
  \multicolumn{1}{l|}{} &
   &
   &
   &
  motivation &
  motivation/not motivational &
  binary \\ \cline{7-9} 
\multirow{-7}{*}{offensive} &
  \multirow{-7}{*}{\textit{Memotion 2 \cite{ramamoorthy2022memotion}}} &
  \multicolumn{1}{l|}{\multirow{-7}{*}{10000 (different ones from Memotion 1)}} &
  \multirow{-7}{*}{Reddit, Facebook, Imgur, Instagram} &
  \multirow{-7}{*}{\textbf{offensive meme detection within meme understanding}} &
  \multirow{-7}{*}{english} &
  modality-class (classification based on) &
  image and text, image, text &
  single-label multi-class \\ \hline
offensive &
  \cellcolor[HTML]{FFFFFF}\textit{MultiOFF \cite{suryawanshi2020multimodal}} &
  743 &
  Reddit, Facebook, Twitter and Instagram., related to U.S. presidential election &
  \textbf{offensive meme detection} &
  english &
  offensiveness &
  yes/no &
  binary \\ \hline
 &
   &
   &
   &
   &
   &
  offensiveness &
  yes/no &
  binary \\ \cline{7-9} 
 &
   &
   &
   &
   &
   &
  explicitness (of offensiveness) &
  implict, explicit &
  binary \\ \cline{7-9} 
 &
   &
   &
   &
   &
   &
  sentiment classification &
  fear, neglect, irritation, rage, disgust, nervousness, shame, disappointment, envy, suffering, sadness, joy, pride, surprise &
  multi-label multi-class \\ \cline{7-9} 
\multirow{-4}{*}{offensive} &
  \multirow{-4}{*}{\textit{Pol\_Off\_Meme \cite{kumari2024enhancing}}} &
  \multirow{-4}{*}{7500} &
  \multirow{-4}{*}{Emoffmeme \cite{kumari2023emoffmeme}} &
  \multirow{-4}{*}{\textbf{offensive meme detection}} &
  \multirow{-4}{*}{hindi} &
  political attributes &
  political/not political &
  binary \\ \hline
offensive &
  \textit{KAU-Memes \cite{bacha2023deep}} &
  2582 &
  Synthetically generated from combining MultiOFF wtih offensive tweets &
  \textbf{offensive meme detection} &
  english &
  offensiveness &
  yes/no &
  binary \\ \hline
offensive &
  \textit{Meme-Merge \cite{alzu2023multimodal}} &
  10000 &
  MET-Meme \cite{xu2022metmeme\}, Memotion 1 \cite{sharma2020semeval\}, Memotion 2 \cite{ramamoorthy2022memotion\} &
  \textbf{offensive meme detection} &
  english &
  offensiveness &
  non-offensiveness, slight, moderate, very-offensive &
  single-label multi-class \\ \hline
offensive &
  \textit{AOMD Gab \cite{shang2021aomd}} &
  1965 &
  Gab &
  \textbf{offensive meme detection} &
  english &
  offensiveness &
  yes/no &
  binary \\ \hline
offensive &
  \textit{AOMD Reddit \cite{shang2021aomd}} &
  1094 &
  Reddit &
  \textbf{offensive meme detection} &
  english &
  offensiveness &
  yes/no &
  binary \\ \hline
propaganda &
  \textit{SemEval-2021 Task 6 \cite{Dimitrov2021detecting}} &
  950 &
  Facebook &
  \textbf{propagandistic technique detection} &
  english &
  propagandistic technique detection &
  Loaded Language, Name Calling/Labeling, Smears, Doubt, Exaggeration/Minimisation, Slogans, Appeal to Fear/Prejudice, Whataboutism, Glittering Generalities, Flag-Waving, Repetition, Causal Oversimplification, Thought-Terminating Cliché, Black-and-White Fallacy/Dictatorship, Straw Man, Appeal to Authority, Reductio ad Hitlerum, Obfuscation, Intentional Vagueness, Confusion, Presenting Irrelevant Data, Bandwagon, Transfer, Appeal to (Strong) Emotions &
  multi-label multi-class \\ \hline
troll &
  \textit{TamilMemes \cite{suryawashi2020dataset}} &
  2969 &
  Whatsapp, Facebook, Instagram, Pinterest &
  \textbf{troll meme detection} &
  tamil &
  troll &
  yes/no &
  binary \\ \hline
 &
   &
   &
   &
   &
   &
  troll/offensiveness &
  yes/no &
  binary \\ \cline{7-9} 
 &
   &
   &
   &
   &
   &
  opinion manipulation &
  yes/no &
  binary \\ \cline{7-9} 
\multirow{-3}{*}{troll, offensiveness} &
  \multirow{-3}{*}{\textit{TrollsWithOpinion \cite{suryawanshi2023trollswithopinion}}} &
  \multirow{-3}{*}{8881} &
  \multirow{-3}{*}{Memotion 1 \cite{sharma2020semeval}} &
  \multirow{-3}{*}{\textbf{troll meme detection}} &
  \multirow{-3}{*}{english} &
  opinion manipulation type &
  political, product, other &
  single-label multi-class \\ \hline
unethical &
  \textit{ELEMENT \cite{zhang2023mvlp}} &
  7912 &
  Google Images, Reddit and Memegenerator &
  \textbf{unethical meme detection} &
  english &
  unethical &
  yes/no &
  binary \\ \hline
 &
   &
   &
   &
   &
   &
  hatefulness &
  yes/no &
  binary \\ \cline{7-9} 
 &
   &
   &
   &
   &
   &
  misogyny &
  yes/no &
  binary \\ \cline{7-9} 
 &
   &
   &
   &
   &
   &
  offensiveness &
  yes/no &
  binary \\ \cline{7-9} 
 &
   &
   &
   &
   &
   &
  sarcasm &
  yes/no &
  binary \\ \cline{7-9} 
\multirow{-5}{*}{hateful, misogynous, offensive, harmful} &
  \multirow{-5}{*}{\textit{GOAT-Bench \cite{lin2024goat}}} &
  \multirow{-5}{*}{6,626} &
  \multirow{-5}{*}{HM, MAMI, MultiOFF, MSD, Harm-C, Harm-P} &
  \multirow{-5}{*}{\textbf{abusive/toxic meme detection}} &
  \multirow{-5}{*}{english} &
  harmfulness &
  yes/no &
  binary \\ \hline
\caption{Meme datasets used by the surveyed works.}
\label{tab:datasets}\\
\end{longtable}

% \cite{hatred} the availability of HatReD enables the exploration of a new
% task, hateful meme explanation. Specifically, we propose a natural language generation task where trained models generate the underlying reasons to explain hateful memes. Such generated reasons can help content moderators better understand the severity and nature of automatically-flagged hateful memes. Similar to [ElSherief et al., 2021], our work can alert the users when they intend to share a particular meme flagged as “hateful” and explain the underlying reasons. This enables
% users to recognize the severity of the hateful meme and possibly reconsider their decision to post the meme. \textbf{introduction of the hateful meme explanation task}

% Evaluation Metrics. We perform both automatic and human evaluations on the baselines. We adopt metrics commonly used in natural language generation tasks for automatic evaluation: (1) N -gram matching for word similarity; and (2) embedding-based metric for semantic similarity. For n-gram matching metrics, we compute the average
% BLEU [Papineni et al., 2002] and ROUGE-L [Lin, 2004]scores. We also compute the harmonic mean of these two
% metrics. We compute the precision, recall, and F1 of the
% BERTScore [Zhang et al., 2019] for embedding-based metric. For human evaluation, we recruit human evaluators to
% assess the generated reasons on two aspects: fluency and relevance. The human evaluators are tasked to rate the generated
% reasons on the Likert scales described in Section 3.1. We also
% mitigate positional bias by presenting the generated reasons
% in a scrambled order.

% \cite{bad}

% \begin{longtable}{|p{7cm}|p{7cm}|}
%         \hline
%         \textbf{Detection Task} & \textbf{Labels} \\
%         \hline
%         Harmfulness \cite{lin2023beneath} & Harmful \\
%                                       & Not harmful \\
%         \hline
%         Intensity of harm \cite{pramanick2021detecting} & Very Harmful \\
%                                                   & Partially Harmful \\
%                                                   & Harmless \\        
        
%         \hline
%         Target of harm: entities type \cite{pramanick2021detecting} & Individual \\
%                                                            & Organization \\
%                                                            & A community \\
%                                                            & Other/Society \\         
%         \hline
%         Specific entity\footnote{specific (person(s), organization(s), and community(ies), e.g., \textit{Barack Obama})} \cite{sharma2022disarm} & Target of harm \\
%                                                         & Not target of harm \\
%         \hline
%         Roles of entities in memes \cite{sharma2022findings} & Hero \\
%                                                                         & Villain \\
%                                                                         & Victim \\
%                                                                         & Other \\
%         \hline
%         Protected categories that are attacked \cite{zia2021racist} & Race \\
%                                                                & Disability \\
%                                                                & Religion \\
%                                                                & Nationality \\
%                                                                & Sex \\
%         \hline
%         Hatefulness \cite{Kiela2020} & Hateful \\
%                                       & Not hateful \\
%         \hline
%         Type of attack \cite{Kiela2020, zia2021racist} & Contempt/Disgust \\
%                                        & Mocking (of disability/of hate crime)\\
%                                        & Inferiority \\
%                                        & Slurs \\
%                                        & Exclusion \\
%                                        & Dehumanizing (comparison to object/animal/criminal) \\
%                                        & Inciting violence \\
%                                        & Negative stereotypes \\
%                                        & Other \\
%         \hline
%         Misogyny manifestations \cite{fersini2019detecting, fersini2021misogynous, fersini2022semeval} & Body shaming \\
%                                                      & Stereotyping \\
%                                                      & Objectification \\
%                                                      & Violence \\
%         \hline
%         Antisemitism types \cite{chandra2021subverting} & Political \\
%                                             & Economic \\
%                                             & Religious \\
%                                             & Racial \\

%         \hline
%         Propagandistic techniques \cite{Dimitrov2021detecting} & Loaded Language \\
%                                                         & Name calling/Labeling \\
%                                                         & Smears \\
%                                                         & Doubt \\
%                                                         & Exaggeration/Minimisation \\
%                                                         & Slogans \\
%                                                         & Appeal to fear/prejudice \\
%                                                         & Whataboutism \\
%                                                         & Glittering generalities (Virtue) \\
%                                                         & Flag-waving \\
%                                                         & Repetition \\
%                                                         & Causal Oversimplification \\
%                                                         & Thought-terminating cliche \\
%                                                         & Black-and-white Fallacy/Dictatorship \\
%                                                         & Straw Man \\
%                                                         & Appeal to authority \\
%                                                         & Reductio ad hitlerum \\
%                                                         & Obfuscation, Int. vagueness, Confusion \\
%                                                         & Presenting Irrelevant Data \\
%                                                         & Bandwagon \\
%         % \hline
%         % Troll meme classification task \cite{suryawanshi2021findings} & Troll \\
%         %                                                         & Not troll \\

%         \hline
%         Fakeness \cite{jabiyev2021game} & ``Fake" meme (containing fake news) \\
%                                       & True meme \\
%         \hline
%         Disinformation \cite{qu2022disinfomeme} & Disinformation meme \\
%                                       & Non-disinformation meme\\
%         \hline
%         Troll with opinion \cite{suryawanshi2021findings} & Non-troll without opinion manipulation \\
%                                       & Non-troll with opinion manipulation\\
%                                       & Troll without opinion manipulation\\
%                                       & Troll with opinion manipulation\\
%         \hline
%     \end{longtable}
%     \label{tab:taxonomy}



% \begin{table}[htbp]
% \renewcommand{\arraystretch}{1.5} % Adjust the vertical padding
% \small
% \resizebox{\linewidth}{!}{%
% \begin{tabular}{|p{3cm}|p{4cm}|p{1cm}|p{1.5cm}|p{5cm}|p{3cm}|} % Adjust the width of the p{} columns as needed
% \hline
% \textbf{Toxicity term} & \textbf{Dataset} & \textbf{By} & \textbf{Magnitude} & \textbf{Derived from} & \textbf{Language} \\ \hline
% cyberbullying &
%   MultiBully &
%   \cite{maity2022multitask} &
%   5854 &
%   Facebook, Twitter, and Reddit &
%   hindi, code-mix \\   \hline

% cyberbullying &
%   MultiBully-Ex &
%   \cite{jha2024meme} &
%   5854 &
%   MultiBully \cite{maity2022multitask} &
%   hindi, code-mix \\  \hline

% derogatory &
%   Derogatory Facebook-Meme &
%   \cite{bhowmick2022multimodal} &
%   650 &
%   Facebook & English, Hindi, and mixed languages \\   \hline

% disinformation &
%   DisinfoMeme &
%   \cite{qu2022disinfomeme} &
%   1170 &
%   Facebook &
%   english \\ \hline
% disinformation/fake &
%   FAME dataset &
%   \cite{jabiyev2021game} &
%   1000 &
%   DuckDuckGo plus Snopes, FactCheck, and PolitiFact &
%   english \\ \hline
% harmful &
%   HarMemes &
%   \cite{pramanick2021detecting} &
%   3544 &
%   \Google Image Search &
%   english \\ \hline
% hateful &
%   Facebook Hateful Memes (HM) &
%   \cite{Kiela2020} &
%   9540 &
%   Artificially constructed from stock photos and designed layouts &
%   english \\ \hline
% hateful &
%   CrisisHateMM &
%   \cite{bhandari2023crisishatemm} &
%   4700 &
%   Twitter, Reddit and &
%   english \\ \hline
% hateful, fine grained &
%   Fine grained FHM &
%   \cite{woah2021} &
%   6000 &
%   FHM &
%   english \\ \hline
% misogynous &
%   Misogynistic-MEME  &
%   \cite{fersini2019detecting, fersini2022misogynous} &
%   800 &
%  Facebook, Twitter, Instagram, and Reddit &
%   english \\ \hline
% misogynous &
%   MAMI (SemEval2022 Task 5, Subtask A) &
%   \cite{fersini2021misogynous} &
%   11000 &
%   Twitter and Reddit &
%   english \\ \hline
% offensiveness &
%   BanglaAbuseMeme &
%   \cite{das2023transfer} &
%   4043 &
%   Google Image SearchBing, Facebook and Instagram &
%   bengali \\ \hline
% offensiveness &
%   Memotion7k &
%   \cite{sharma2020semeval} &
%   6992 &
%   Google Image Search &
%   english \\ \hline
% offensiveness &
%   MultiOFF &
%   \cite{suryawanshi2020multimodal} &
%   743 &
%   Reddit, Facebook, Twitter and Instagram &
%   english \\ \hline
% offensiveness &
%   Emoffmeme &
%   \cite{kumari2023emoffmeme} &
%   7500 &
%   Google Image Search &
%   hindi \\  \hline
% offensiveness &
%   Pol\_Off\_Meme &
%   \cite{kumari2024enhancing} &
%   7500 &
%   Emoffmeme \cite{kumari2023emoffmeme} &
%   hindi \\  \hline
% offensiveness, fine-grained &
%   Titli et al &
%   \cite{titli2023automated} &
%   15636 &
%   Multi-modal Hate Speech Bengal \cite{karim2022multimodal} and Bengali Hate Speech \cite{romim2021hate} &
%   bengali \\  \hline
% propagandistic techniques &
%   SemEval-2021 Task 6 &
%   \cite{Dimitrov2021detecting} &
%   950 &
%   Facebook groups &
%   english \\ \hline
% roles in harmful &
%   HVVMemes &
%   \cite{sharma2022findings} &
%   7000 &
%   HarMemes \cite{pramanick2021detecting} &
%   english \\ \hline
% troll &
%   TrollsWithOpinion &
%   \cite{suryawanshi2023trollswithopinion} &
%   8881 &
%   Memotion \cite{sharma2020semeval} &
%   english \\ \hline
% unethical &
%   ELEMENT &
%   \cite{zhang2023mvlp} &
%   7912 &
%   Google Image Search, Reddit and Memegenerator &
%   english \\
%   \bottomrule
% \end{tabular}
% }
% \caption{Meme datasets used by the surveyed works, classified by toxicity type, magnitude, and where the memes come from, language}
% \label{tab:datasets}
% \end{table}


% % for misogyny:

% % Dataset	Used by
% % SemEval-2022 MAMI Challenge Dataset	Chen et al. \cite{chen2022rit}, Kalkenings et al. \cite{kalkenings2022university}, Paraschiv et al. \cite{paraschiv2022upb}
% % MAMI Dataset	Behzadi et al. \cite{behzadi2022mitra}
% % Facebook Hateful Memes Challenge Dataset	Kalkenings et al. \cite{kalkenings2022university}
% % Explainable Detection of Online Sexism Challenge Dataset	Obeidat et al. \cite{obeidat2023just_one}

% % Architectural Method	Utilized by
% % Perceiver IO	Attanasio et al.
% % CLIP (Contrastive Language-Image Pre-training)	Behzadi et al., Chen et al., Paraschiv et al., Singh et al.
% % BERT (Bidirectional Encoder Representations from Transformers)	Obeidat et al., Paraschiv et al., Singh et al.
% % VisualBERT	Fersini et al., Ravagli et al., Singh et al.
% % Mask R-CNN	Ravagli et al.
% % Variational AutoEncoder (VAE)	Gu et al.
